Double layer in ionic liquids: capacitance vs temperature

Temperature dependence of the capacitance of the electrical double layer (EDL) in concentrated electrolytes/ionic liquids has been under debates for decades. To rationalise the capacitance vs temperature dependence, we run molecular dynamics simulations of the EDL at variable temperatures. We show that the dependence is related to the smearing of the EDL multilayer structure with increasing temperature. The results are in agreement with the recent experimental data. To explain the results, we propose a phenomenological ionic bilayer model.

==> Reviewers.tex <==
Reviewer #1 Evaluations: 
Recommendation: Major revision 
New Potential Energy Surface: No 

Reviewer #1 (Comments to the Author): 

This article reports some interesting findings on the impact of temperature on the double-layer capacitance. However, I think several aspects need to be carefully addressed before publication in the Journal of Chemical Physics. 

From the technical point of view: 
1/ It seems that the simulations were performed at the same volume for all the temperatures, however in experiments there should be a large expansion between 250 K and 500 K. Did the authors try to account for this? 
2/ I do not see any argument for scaling the charges by the square root of two. Why did the authors do that? Is there an interest since anyway they use a primitive model which is not supposed to mimic any real ionic liquid? 
3/ The vacuum layer seems very small. In many studies of slab systems it was shown that taking a layer of vacuum which is 3 to 5 times larger than the layer of liquid is necessary. Did the authors do any test for the present study? 

Now concerning the results: 
1/ I do not understand the statement "Eq. 1 is valid only if C is independent on the potential" (page 4). I rather think that this equation is never valid for a liquid electrolyte (or maybe at infinite dilution) since it is not possible to measure (or even to define) epsilon and the distance. 
2/ Can the authors specify what they mean when they define Delta below equation 3? Here it seems that it is the distance within the ith layer, but based on the discussion it should rather be between two successive layers. Or maybe I have misunderstood? 
3/ Please correct "anamalous" (appears several times) 
4/ I think the authors should provide the anion density profile somewhere, showing the positions of the layers is not enough. In particular it would be necessary to see whether the first layer of cations also contains many anions. 
5/ In the caption of Fig. 2 there is a typo for panels c) and d), the potential should be different. 
6/ if I understand well Figure 3e), the first peak intensity grows continuously? Shouldn't there be a saturation in the number of anions. 
7/ Based on the comparison between Figures 3d and 3e it seems to me that much more cations could be packed in the second layer. Then is it accurate to say that a dense layer is obtained? 
8/ I am not sure why CN1+CN2=-sigma A (what are CN1 and CN2? If they correspond to anions and cations shouldn't there be a minus sign somewhere?) 
9/ The authors should expand the calcution which gives the result provided in equation 4 
10/ The denominator in equation 5 does not seem to be homogeneous. 
11/ What is the "potential of maximum entropy"? The last sentence before the conclusions should either be removed or explained better. 


Reviewer #2 Evaluations: 
Recommendation: Reject 
New Potential Energy Surface: No 

Reviewer #2 (Comments to the Author): 

This manuscript presents a classical molecular dynamics study of the double layer capacitance dependence on temperature and proposes a model to explain the dependence observed. While I think the topic is timely and relevant for energy storage, my recommendation for this manuscript is to reject it. I think that this work is not suitable for the Journal of Chemical Physics as there are a number of important problems. The points that I think are the most important flaws are listed below. 

- In the last part of the manuscript before the conclusions, the authors propose a phenomenological ionic bilayer model to explain the capacitance dependence. While the approach is interesting according to the undertaken MD study, it does not seem to me that the authors actually test their model. They provide equations (Eq. 4 and Eq. 5) but they do not compare the values which would be obtained through these equations to the MD simulations whereas they should have all the information to do it. If not quantitative values, they could show qualitative trends. As such, it is difficult to assess the validity of the model and to follow the two paragraphs starting from "Using the ionic bilayer model [...]" and "The maximal charge excess [...]" on page 7-8. The results would be rendered much stronger if the model would be used to predict capacitance dependences of other "ionic liquids", for example for different ion sizes and to check these assumptions with MD by changing the ion sizes in the simulations. The simplicity of the liquid model is ideally suited for this kind of study. Overall, it seems that the study is incomplete. 

- One other point I have problems with is the model for the "ionic liquid" and the simulation system studied. On this, I have three main concerns. 
1) The authors explain that they build a system with 1050 ions pairs in a simulation box where the accessible volume is 2900 nm3: this corresponds to a molar concentration of approximately 0.6M which is quite a bit lower than the usual concentration of pure ionic liquids. Indeed, ionic liquids, even with larger ion sizes, have molar concentrations around 4.4M (BMI-PF6), 3.6M (P13TFSI), 4.4M (P13FSI) to give only a few examples. Do the authors have an idea of the influence of this on the capacitance of the double layer. It is for example easy to see that for neutral or charge surfaces, the ionic densities in the first layer adsorbed on the electrodes are systematically lower in this work compared to other more realistic systems: ionic densities around 1.0-1.3 nm-3 are reported in this paper (Fig. 2) against i) 8.0-14.0 nm-3 (TFSI) and 8.0-28.0 nm-3 (Pyr13) for the ionic liquid in ref 22, ii) 18.0-33.0 nm-3 (PF6-) and 10.0-18.0 nm-3 (BMI+) for the ionic liquid in ref 24. If the authors are confident in the suitability of their model, they should at least comment on this. 
2) On top of the small densities, the authors use a dielectric constant not equal to 1 but rather to 2. This tends to reduce the electrostatic interactions and is indeed quite commonly used in simulations of ionic liquids, usually written as ions having a charge lower than 1e. But this is usually used for normally concentrated systems of around 4-5M and using charges of 0.8e (for example, see ref 25) which would lead to a dielectric constant of 1.5625 (~20% smaller than 2.0). 
-> So with points 1) and 2) together, the electrostatic interactions between ions are really largely reduced in this work compared to realistic systems and it would probably be necessary to investigate the effect of this on the capacitance in general and also its dependence with temperature. 
3) The last point is about the potential itself. The authors choose to work with a simple Lennard-Jones repulsive potential. I am curious why the choice of not using the dispersion part was made and how this impacts the structure and dynamics of the double layer. 

- A maybe less crucial point is the use of constant charges on the electrode walls to simulate experimental systems with metallic electrodes. This is a well known issue in the field. Constant charges (for which calculations are much faster) have shown to reproduce well the structure of the double layer in some cases but dynamical properties not so well. As for the temperature dependence, the use of constant potential / constant charge on the electrodes might have an influence. This should probably be at least commented on if not tested. In the manuscript in its current form, the authors could put a curve to show the relation between potential and surface charge. There are points where the "equivalence" is noted in parentheses but in other places, the figures interpretation is hard to follow because the text mentions potentials while the figures show surface charges. Also, the authors write "The effective charge used in the simulations was obtained by scaling the "physical" charge by 1/√2". It is not clear to me why this was done. 

In my opinion, each of these points taken separately might not be enough to reject the paper but the accumulation of these issues makes it hard to see the achievements / originalities of this work, and more importantly, the specificities of the model makes one doubt about the solidity of the conclusions for a pure ionic liquid (as the system tends to look like a solvated electrolyte). 


Answers:

Thank you very much for resenting the review's comments to the Manuscript No.: ILQ17.11.0193.

The questions of the first reviewer can be quickly addressed. 1. We should have written in the methods section that the density was varied with the temperature. 2. A typical refractive index value is 1.4, which corresponds to eps = 2.0. 3. Others may not apply the dipole correction, so they do have to add a wide vacuum layer. Perhaps, authors of Ref 25 did not used the dipole correction, as there is a bug in Gromacs 4.6.x. We used Gromacs 4.5.5 and did numerous tests. In Gromacs 2016 there is way to skip the vacuum layer at all.

I agree with the second review that the analyses can be improved. We will extended it along with the discussion prior the next submission. As for the criticism of the model, let me just point that, firstly, there are ionic liquids with the ionic density below 1 M,* and, secondly, polarizability in ionic liquid models and constant-potential-simulations are not the same. Luckily, as the paper is rejected there is no need to argue.

Please resent this letter to the reviews. Dear all, thank you very much for taking your time to review the manuscript!

Withing you a Merry Christmas and a Happy New Year,
Vladislav Ivaništšev

* e.g. ionic density of trihexyl(tetradecyl)-phosphonium tris(pentafluoroethyl) trifluorophosphate is ~0.76 M. The size of the ions is comparable to our model, yet treir packing in the real liquid is more dense due to the complex molecular shape in comparison to simple spheres.
